Evaluation of Quantum Machine Learning Models for Network Anomaly Detection

The proliferation of Internet-connected devices has intensified the risk of large-scale network intrusions, necessitating more advanced detection methodologies for the post quantum era. This work presents, to the best of our knowledge, a com- prehensive investigation of quantum machine learning (QML) for anomaly detection on the BoT-IoT dataset, a widely adopted benchmark for IoT security. Leveraging feature-engineered rep- resentations, we implement and evaluate four representative quantum classifiers: Quantum Support Vector Classification (QSVC), Quantum Neural Networks (QNN), and Variational Quantum Classifiers (VQC).

==> extra.tex <==
\subsection{Availability of a Laser Inter-Satellite Link (ISL)}

Consider satellites $i$ and $j$. Let $T$ be a reference period (e.g., one orbital repeat).
Define the binary \emph{link-existence} indicator
\[
\mathbb{I}_{ij}(t)\;=\;
\underbrace{\mathbb{I}_{\mathrm{LOS}}(t)}_{\text{geometric line-of-sight}}
\cdot
\underbrace{\mathbb{I}_{\mathrm{AER}}(t)}_{\text{elevation (and optional pointing) limits}}
\cdot
\underbrace{\mathbb{I}_{\mathrm{policy}}(t)}_{\text{pairing/scheduling policy}},
\]
and the \emph{geometric availability} of link $(i,j)$ over $[0,T]$ as
\begin{equation}
A_{ij}^{\mathrm{geo}}
\;=\;
\frac{1}{T}\int_{0}^{T}\mathbb{I}_{ij}(t)\,dt.
\label{eq:Aij_def}
\end{equation}

\paragraph{Geometry and LOS test}
Let $(\varphi_k(t),\lambda_k(t))$ be the latitude/longitude of satellite $k\in\{i,j\}$,
with geocentric angle
\begin{equation}
\theta(t)
=
\arccos\!\big[\sin\varphi_i\,\sin\varphi_j+\cos\varphi_i\,\cos\varphi_j\cos(\lambda_i-\lambda_j)\big].
\label{eq:theta}
\end{equation}
(Orbital kinematics for $(\varphi,\lambda)$ follow the paper’s Eqs.\,(8)–(10).) Given
orbital radii $R_i,R_j$, the instantaneous separation and elevation angles are
\begin{align}
d_{ij}(t) &= \sqrt{R_i^2+R_j^2-2R_iR_j\cos\theta(t)}, \label{eq:dij}\\
\delta_i(t) &= \arccos\!\Big(\tfrac{R_j\sin\theta(t)}{d_{ij}(t)}\Big),\quad
\delta_j(t) = \arccos\!\Big(\tfrac{R_i\sin\theta(t)}{d_{ij}(t)}\Big). \label{eq:deltaij}
\end{align}
Define $h_i'(t)=R_i\cos\delta_i(t)$. With atmospheric thickness $H$ and Earth
radius $R$, the paper’s visibility criterion is
\begin{equation}
\mathbb{I}_{\mathrm{LOS}}(t)=
\begin{cases}
1,& \text{if } h_i'(t)>R+H \ \ \text{or}\ \ d_{ij}(t)<x,\\
0,& \text{otherwise,}
\end{cases}
\qquad
x=2\sqrt{R_i^2-(R+H)^2}.
\label{eq:los_test}
\end{equation}
For co-orbital neighbors with constant relative geometry, the simpler Earth-occlusion
test $(R+h)\cos\gamma > (R+H)$ applies.  % paper Eq.(6)
Optionally enforce minimum elevation $\delta_{\min}$ at both ends via
\begin{equation}
\mathbb{I}_{\mathrm{AER}}(t)=\mathbb{I}\{\delta_i(t)\ge \delta_{\min}\}
\cdot\mathbb{I}\{\delta_j(t)\ge \delta_{\min}\}.
\label{eq:aer_gate}
\end{equation}

\paragraph{Pairing/scheduling policy (capacity of terminals)}
If a node can simultaneously maintain only a limited number of LISLs (e.g., four
terminals per Starlink satellite), include a policy gate $\mathbb{I}_{\mathrm{policy}}(t)\in\{0,1\}$
that reflects the topology rule (e.g., fixed pairs with two co-orbital neighbors and
adjacent-plane neighbors).  % per paper's link policy
This converts purely geometric availability in \eqref{eq:Aij_def} into \emph{operational}
availability:
\begin{equation}
A_{ij}^{\mathrm{op}}=\frac{1}{T}\int_{0}^{T}\mathbb{I}_{\mathrm{LOS}}(t)\,\mathbb{I}_{\mathrm{AER}}(t)\,
\mathbb{I}_{\mathrm{policy}}(t)\,dt.
\label{eq:Aij_op}
\end{equation}

\paragraph{Classification implied by the model}
If $\mathbb{I}_{ij}(t)=1$ for all $t\in[0,T]$, the link is \emph{permanently visible} 
($A_{ij}^{\mathrm{op}}=1$). Otherwise it is \emph{intermittently visible}, and
$A_{ij}^{\mathrm{op}}$ equals the fraction of time the LOS and AER constraints hold under
the chosen pairing policy.


\color{blue}

 Incorporating link availability $\alpha_k(t)$, protocol and framing overheads $\theta_k(t)$, and terminal utilization $u_k(t)$, the node capacity can be written as
\begin{equation}
C_{\text{node}}(t) = \sum_{k=1}^{d} \alpha_{k}(t)\,\big(1 - \theta_{k}(t)\big)\,u_{k}(t)\,C_{\text{ISL},k}(t).
\label{eq:node_capacity}
\end{equation}

Here, $\alpha_{k}(t)$ reflects the duty cycle of each terminal considering acquisition and handover interruptions, $\theta_{k}(t)$ captures the overhead fraction from FEC, framing, and routing, $u_{k}(t)$ represents the utilization factor of the $k$-th terminal, and $C_{\text{ISL},k}(t)$ is the instantaneous Shannon capacity of the respective ISL. 



% considering the transmission bandwidth of $B^{s}$ and the noise component~($N_{\mathrm{th}}^{s}$), capacity of the link~($C_{\mathrm{S}}(t)$) can be modeled as:
% \begin{equation}
% C_{\mathrm{S}}(t)
% \;=\;
% B^{s} \,\log_2\!\left(1+\frac{P_\mathrm{r}^{s}(t)}{N_{\mathrm{th}}^{s}}\right).
% \label{eq:isl_capacity_final}
% \end{equation}


% \color{blue}
% \subsection{Impact of SNR Variance on Modulation Capability Under ACM}


% Let the probability of selecting MCS $k$ be
% \begin{equation}
%     p_k = \mathbb{P}\left(\tau_{k-1} \leq \gamma < \tau_{k}\right) 
%         = F_{\gamma}(\tau_{k}) - F_{\gamma}(\tau_{k-1}),
% \end{equation}
% where $F_{\gamma}(\cdot)$ is the cumulative distribution function (CDF) of $\gamma$. 
% The expected spectral efficiency under ACM is therefore
% \begin{equation}
%     \mathbb{E}[\eta] = \sum_{k=1}^{K} \log_{2} M_k \cdot r_k \, p_k,
% \end{equation}
% and the variance is
% \begin{equation}
%     \mathrm{Var}[\eta] = \sum_{k=1}^{K} \left(\log_{2} M_k \cdot r_k \right)^{2} p_k
%     - \left( \sum_{k=1}^{K} \log_{2} M_k \cdot r_k \, p_k \right)^{2}.
% \end{equation}

% \subsubsection{Direct Link Between SNR and Modulation Variance}
% The probabilities $\{p_k\}$ depend solely on the distribution of $\gamma$, which is shaped by its variance $\sigma_{\gamma}^2$. When $\sigma_{\gamma}^2$ is small, $\gamma$ remains concentrated around $\mu_{\gamma}$, so most probability mass lies in a single interval $[\tau_{k-1}, \tau_{k})$, and ACM selects a single MCS with high certainty. In this case, $\mathrm{Var}[\eta] \approx 0$. Conversely, when $\sigma_{\gamma}^2$ is large, $\gamma$ spreads across multiple thresholds, causing ACM to switch between several MCS levels. This directly increases $\mathrm{Var}[\eta]$, reflecting a higher variability in achievable modulation capability. 

% Formally, we express this dependence as
% \begin{equation}
%     \mathrm{Var}[\eta] = \mathcal{F}(\sigma_{\gamma}^2),
% \end{equation}
% where the functional $\mathcal{F}(\cdot)$ is determined by the ACM threshold set $\{\tau_k\}$ and the underlying SNR distribution $f_{\gamma}(\cdot)$. 

% \subsubsection{Implications for Starlink}
% In a Starlink downlink, the distribution of $\gamma(t)$ broadens due to orbital dynamics and atmospheric fading. As a direct consequence, ACM must frequently adapt between QPSK, 16-QAM, and 64-QAM modes, thereby increasing $\mathrm{Var}[\eta]$. This variance manifests in practice as fluctuations in user throughput. Thus, the modulation variance observed at the receiver is not an independent phenomenon but is a deterministic projection of the underlying SNR variance through the ACM mechanism. 


% \subsubsection{Effect of Modulation Variance on Capacity}


% From \eqref{5}, the mean capacity is
% \begin{equation}
%     \mathbb{E}[C] = B \cdot \mathbb{E}[\eta] 
%     = B \sum_{k=1}^{K} \log_{2} M_k \cdot r_k \, p_k,
% \end{equation}
% and the variance of the capacity is
% \begin{equation}
%     \mathrm{Var}[C] = B^{2} \, \mathrm{Var}[\eta].
% \end{equation}

% Equations (9)–(11) demonstrate that the variability of the achievable modulation directly scales into the variability of the instantaneous capacity. 


\begin{comment}
Starlink satellites move in their orbits at approximately $7.5~\mathrm{km/s}$. 
Therefore, from the perspective of a ground user, the slant range and the elevation angle vary continuously with time. 
Consequently, free-space path loss $L_\mathrm{fs}^{s}(t)$ is inherently time-dependent. 
In addition, the pointing directions of the satellite phased array and the user terminal phased array evolve during the satellite pass, resulting in variations in the antenna gain terms. 
Therefore, the link margin $M(t)$, defined as the difference between the received \gls{snr}~($SNR^{S}(t)$) and the required threshold~($SNR_{req}$) becomes a function of time.

Since each satellite is visible for only a short duration, depending on the elevation cutoff angle, the user terminal must switch to a new satellite before the current one descends below the visibility mask. 
Modern phased-array user terminals enable \gls{mbb} handovers by forming two simultaneous beams, one maintains the link with the current satellite $j_\mathrm{prev}$, while the other establishes a link to the next satellite $j_\mathrm{next}$. 

The serving satellite index at time $t$ can be modeled as
\begin{equation}
    j^\star(t) = \arg\max_{j \in \mathcal{S}(t)} 
    \left\{ M_j(t) - \mathbb{I}_{\{j \neq j^\star(t^-)\}} H \right\},
\end{equation}
where $\mathcal{S}(t)$ is the set of satellites above the minimum elevation angle, $M_j(t)$ is the link margin with satellite $j$, and $H$ is a hysteresis margin introduced to prevent frequent handover oscillations. 


The availability of a LEO satellite communication link can be defined as the fraction of time during which the link margin remains above the required threshold. 
Outages may occur if (i) no satellites are above the elevation mask, (ii) atmospheric fading due to rain, clouds, or scintillation degrades the link below threshold, or (iii) the handover process fails.

Thus, we define an outage indicator function as
\begin{equation}
    \mathbb{I}_{out}(t) = 
    \begin{cases}
        1, & \max\limits_{j \in \mathcal{S}(t)} M_j(t) < 0, \\
        0, & \text{otherwise},
    \end{cases}
\end{equation}
Accordingly, the availability over a time horizon $[0,T]$ is expressed as
\begin{equation}
    \mathcal{A} = \frac{1}{T} \int_0^T 
    \mathbb{I}\!\left( \max_{j \in \mathcal{S}(t)} M_j(t) \geq 0 \right) dt.
\end{equation}

With \gls{mbb} handovers, the availability remains close to $100\%$, since handover gaps are effectively suppressed. 
In contrast, \gls{bbm} handovers reduce availability slightly at each switching event. 
\end{comment}


\begin{comment} 
\paragraph{Network Bottleneck Analysis}

For multi-hop connections, data transfer may traverse $n$ \glspl{isl}. In such cases, the effective service rate is limited by the minimum \gls{isl} capacity along the selected path, denoted as $\min_{i \in \{1,2,\dots,n\}} \big[ C_{\text{ISL},i}(t) \big]$
Thus, the end-to-end user throughput is bounded by the minimum of multiple constraints, the satellite to ground terminal link capacity ($C_{\mathrm{S}}(t)$), the weakest \gls{isl} on the path, the \gls{cca}-driven sending rate ($T_{\text{CCA}}(t)$).   
This can be formalized as
\begin{equation}
T(t) = \min \Big\{ C_{\mathrm{S}}(t), \; \min_{i \in \{1,\dots,n\}} \big[ C_{\text{ISL},i}(t) \big], \; T_{\text{CCA}}(t)\Big\}
\label{eq:throughput}
\end{equation}
For simplicity, we are assuming that the other systemic bottlenecks, such as optical switch fabric limits, routing inefficiencies, and application-layer rate constraints, are not causing any bottlenecks.

\end{comment}



\begin{comment}
    

In the uplink experiments across the globally distributed locations, \gls{bbr} consistently achieved the highest throughput for all six locations, upper whiskers exceeding $80$ Mbps in some cases (Fig.~\ref{fig.upload_box}(a), ~\ref{fig.uplink_time}(a) and (d)). 
This stems from \gls{bbr}’s model-based pacing, which estimates the bottleneck bandwidth and \gls{rtt} to fill the pipe efficiently, unlike loss-based \glspl{cca} such as Cubic or Hybla, thus resulting in higher variance. 
Hybla achieved throughput improvements in moderately high-\gls{rtt} paths such as Tokyo, Mumbai, due to its \gls{rtt} compensation mechanism, but it was still significantly below \gls{bbr}. 
Vegas and Cubic remained throughput-limited, rarely exceeding 10 Mbps, constrained by their conservative congestion avoidance and delay-based growth, respectively. 
Since throughput $T \approx \frac{\text{cwnd}}{\text{RTT}}$, \gls{bbr} maintains a much higher congestion window (Fig.~\ref{fig.upload_box}c) relative to the \gls{rtt} (Fig.~\ref{fig.upload_box}(c), Fig.~\ref{fig.uplink_time}(b) and (e)), thereby yielding superior throughput.

Retransmission behavior as depicted in Fig.~\ref{fig.upload_box}(b) highlights the cost of \gls{bbr}'s aggressiveness. 
While \gls{bbr} achieve comparatively the highest congestion window values ($Q_2 < 0.4$MB), this resulted in significantly higher retransmission counts with $Q_2$ < $10$--$25$ packets, with upper tails exceeding $70$ packets in some locations. 
In contrast, Cubic and Vegas showed retransmission counts typically below $5$, reflecting their more cautious probing of available bandwidth. 
Hybla displayed intermediate retransmission levels, balancing aggressive congestion window inflation against \gls{rtt} compensation. 
The receiver-advertised window is generally stable around $4$--$5$MB (Fig.~\ref{fig.upload_box}(d)), indicating that the sender-side algorithm, rather than receiver-side constraints, dictated performance. 
This suggests that \gls{bbr} tends to operate closer to the link’s actual capacity, albeit at the expense of elevated packet loss and retransmission overhead.

\gls{rtt} and \gls{rtt} variance (Fig.~\ref{fig.upload_box}(e), \ref{fig.upload_box}(f), ~\ref{fig.uplink_time}(c) and ~\ref{fig.uplink_time}(f)) confirm Starlink’s latency heterogeneity across geographies. 
São Paulo exhibited the highest RTTs ($>300$ ms), consistent with longer ground-satellite-gateway paths, while Sydney showed the lowest ($Q_2 \approx 50$ ms). 
The delay variance remained comparatively similar across all \glspl{cca}, a signature of improved LEO handover dynamics and queue variability in Starlink network. 
Hybla’s \gls{rtt}-independent scaling allowed it to achieve higher throughput in high-delay paths compared to Cubic and Vegas, but it still could not match for aggressiveness in \gls{bbr}, which explicitly decouples its sending rate from packet loss events. 
Overall, the results reinforce that while $T \propto \tfrac{1}{\text{RTT}}$ in Reno-like \glspl{cca}, Hybla mitigates this proportionality via scaling, and \gls{bbr} bypasses it entirely by maintaining a \gls{bdp} estimate, making it the most productive algorithm for Starlink’s dynamic LEO environment.
\end{comment}


\begin{comment}
    
\gls{bbr} achieved the highest throughput across all six locations in the downlink experiments, with median values frequently exceeding $150$~Mbps and peaks approaching $350$~Mbps in some regions (Fig.~\ref{fig.download box}(a), \ref{fig.downlink_time}(a) and (d)). 
This superior performance arises from \gls{bbr}'s proactive model-driven congestion control, which fills the \gls{bdp} without waiting for packet losses. 
In comparison, Hybla and Cubic achieved moderate throughput in the range of $Q_2 \approx 20$--$60$~Mbps, while Vegas was significantly limited, rarely exceeding $10$~Mbps. 
This is primarily achieved through \gls{bbr}'s higher congestion window (Fig.~\ref{fig.download box}(c), \ref{fig.downlink_time}(b) and (e)) enables much larger sending rates for similar \gls{rtt} compared to other \glspl{cca}.  

The retransmission patterns (Fig.~\ref{fig.download box}(b)) underline the trade-off of \gls{bbr}'s aggressiveness. 
Tokyo and Mumbai, in particular, exhibited retransmission counts exceeding $300$ packets, an order of magnitude larger than the negligible retransmissions observed for Cubic, Hybla, and Vegas. 
This suggests that \gls{bbr} probes the link more aggressively, overshooting capacity during satellite handovers and queue variations, which induces losses. 
Nonetheless, the receiver-advertised window (Fig.~\ref{fig.download box}(d)) remained consistently high and steady, confirming that receiver-side constraints were not a bottleneck. 
Hence, the elevated retransmissions are attributable to \gls{bbr}’s sender dynamics rather than flow-control limitations.  

\gls{rtt} and its variance provide additional insights into performance. 
São Paulo again showed the highest \glspl{rtt} ($>350$~ms), while Sydney exhibited the lowest values ($<80$~ms), consistent with geographic proximity to gateways (Fig.~\ref{fig.download box}(e), \ref{fig.downlink_time}(b) and \ref{fig.downlink_time}(e)). 
The \gls{rtt} variance across all \glspl{cca}  remained within $2$--$8$~ms (Fig.~\ref{fig.download box}(f), \ref{fig.downlink_time}(c) and \ref{fig.downlink_time}(f)), indicating that Starlink’s LEO handover dynamics impose a relatively stable but non-negligible jitter. 
Hybla demonstrated resilience in high-\gls{rtt} environments due to its scaling factor $\rho = RTT/RTT_0$, which compensates for delay, but still underperformed relative to \gls{bbr}. 
Overall, the results highlight that \gls{bbr} maximizes throughput in Starlink’s variable downlink conditions by explicitly targeting the \gls{bdp}, whereas traditional loss and delay-based \glspl{cca} maintain conservative sending rates, achieving stability at the cost of under-utilizing available capacity.

    
\noindent\begin{observation}[BBR-v3 Throughput Dominance with Higher Loss Cost]
Across all six global endpoints and in both uplink and downlink directions, BBR-v3 consistently achieved the highest throughput among the evaluated CCAs (Cubic, Hybla, Vegas). Median downlink rates frequently exceeded 150~Mbps, with peaks approaching 350~Mbps in some regions, while uplink medians were markedly higher than competing CCAs. This performance correlates with BBR-v3's higher congestion window and model-based pacing that targets the bottleneck BDP.
\end{observation}

\noindent\begin{finding}
The throughput gains of BBR-v3 come at the cost of increased retransmissions—particularly pronounced during downlink to Tokyo and Mumbai, where retransmission counts exceeded 300 packets—suggesting aggressive probing overshoots capacity during satellite handovers and queue fluctuations. Receiver-advertised windows remained stable (typically 4--5~MB), indicating that elevated losses stem from sender dynamics rather than flow-control limitations.
\end{finding}
\end{comment}

